A Novel Stochastic Gradient Descent Algorithm for Learning Principal Subspaces

Many machine learning problems encode their data as a matrix with a possibly very large number of rows and columns. In several applications like neuroscience, image compression or deep reinforcement learning, the principal subspace of such a matrix provides a useful, low-dimensional representation of individual data. Here, we are interested in determining the $d$-dimensional principal subspace of a given matrix from sample entries, i.e. from small random submatrices. Although a number of sample-based methods exist for this problem (e.g. Oja's rule \citep{oja1982simplified}), these assume access to full columns of the matrix or particular matrix structure such as symmetry and cannot be combined as-is with neural networks \citep{baldi1989neural}. In this paper, we derive an algorithm that learns a principal subspace from sample entries, can be applied when the approximate subspace is represented by a neural network, and hence can be scaled to datasets with an effectively infinite number of rows and columns. Our method consists in defining a loss function whose minimizer is the desired principal subspace, and constructing a gradient estimate of this loss whose bias can be controlled. We complement our theoretical analysis with a series of experiments on synthetic matrices, the MNIST dataset \citep{lecun2010mnist} and the reinforcement learning domain PuddleWorld \citep{sutton1995generalization} demonstrating the usefulness of our approach.

==> defs.tex <==

\usepackage[utf8]{inputenc} %
\usepackage[T1]{fontenc}    %
\usepackage{hyperref}       %
\usepackage{url}            %
\usepackage{booktabs}       %
\usepackage{amsfonts}       %
\usepackage{nicefrac}       %
\usepackage{microtype}      %
\usepackage{xcolor}         %
\usepackage[framemethod=TikZ]{mdframed}
\usepackage{hyperref}
\usepackage{url}
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{subcaption}
\usepackage{booktabs} %
\usepackage{bbm}
\usepackage{hyperref}
\usepackage[nameinlink,capitalise]{cleveref}
\crefname{figure}{Figure}{Figures}
\Crefname{figure}{Figure}{Figures}
\crefname{table}{Table}{Tables}
\Crefname{table}{Table}{Tables}
\crefname{equation}{Equation}{Equations}
\Crefname{equation}{Equation}{Equations}
\crefname{section}{Section}{Sections}
\Crefname{section}{Section}{Sections}
\crefname{subsection}{Subsection}{Subsections}
\Crefname{subsection}{Subsection}{Subsections}
\usepackage{wrapfig} 
\usepackage{microtype}
\usepackage{booktabs} %
\usepackage{wrapfig}
\usepackage{algorithm}
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{amsthm}
\usepackage{stmaryrd}
\usepackage{mathtools}
\usepackage{bm}
\usepackage{dblfloatfix}
\usepackage{enumitem}
\usepackage[thinc]{esdiff}
\usepackage{bigints}
\usepackage{mdwlist}
\usepackage{thmtools, thm-restate}
\usepackage{pgfplots}
\usepackage{makecell}


\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{lemmaap}{Lemma}
\renewcommand*{\thelemmaap}{\Alph{lemmaap}}
\newtheorem*{remark}{Lemma}
\declaretheorem{proposition}
\declaretheorem{property}
\declaretheorem{corollary}
\declaretheorem{definition}
\declaretheorem[numbered=no]{principle}
\usepackage{amsmath}
\usepackage{centernot}
\newtheorem{innercustomthm}{Theorem}
\newenvironment{customthm}[1]
  {\renewcommand\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}
\newtheorem{innercustomlemma}{Lemma}
\newenvironment{customlemma}[1]
  {\renewcommand\theinnercustomlemma{#1}\innercustomlemma}
  {\endinnercustomlemma}
\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\opnorm}[1]{\norm{#1}_{\mathrm{op}}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\T}{\mathsf{T}}

\usepackage{tikz-cd}

\renewcommand{\ge}{\geqslant}
\renewcommand{\geq}{\geqslant}
\renewcommand{\le}{\leqslant}
\renewcommand{\leq}{\leqslant}
\renewcommand{\preceq}{\preccurlyeq}
\renewcommand{\succeq}{\succcurlyeq}

\newcommand{\deff}{d_{\mathrm{eff}}}
\newcommand{\unorm}[1]{\lVert #1 \rVert_{S, 2}}
\newcommand{\bignorm}[1]{\left\lVert #1 \right\rVert}
\newcommand{\twonorm}[1]{\lVert #1 \rVert_{2}}
\newcommand{\maxnorm}[1]{\lVert #1 \rVert_{\infty}}
\newcommand{\onenorm}[1]{\left\lVert #1 \right\rVert_{1}}
\newcommand{\mb}[1]{\mathbf{#1}}
\newcommand{\bigip}[2]{\ensuremath{\left\langle #1, #2 \right\rangle}}
\newcommand{\ip}[2]{\ensuremath{\langle #1, #2 \rangle}}
\newcommand{\PD}[2]{\ensuremath{\frac{\partial #1}{\partial #2}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\abs}[1]{\ensuremath{| #1 |}}
\newcommand{\bigabs}[1]{\ensuremath{\left| #1 \right|}}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\bigfloor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\Normal}{\mathcal{N}}
\newcommand{\rdraw}{\xleftarrow{\$}}
\newcommand{\ind}{\mathbf{1}}
\renewcommand{\vec}{\mathrm{vec}}
\newcommand{\Sym}{\mathbf{S}}
\renewcommand{\Re}{\mathrm{Re}}
\renewcommand{\Im}{\mathrm{Im}}
\DeclareMathOperator*{\Tr}{\mathrm{tr}}
\newcommand{\TxM}{\mathcal{T}_x\mathcal{M}}
\newcommand{\TxtM}{\mathcal{T}_{x(t)}\mathcal{M}}
\newcommand{\leb}{\mu}
\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\TM}{\mathcal{TM}}
\newcommand{\TTM}{\mathcal{TTM}}
\newcommand{\smax}{\sigma_{\mathrm{max}}}
\newcommand{\smin}{\sigma_{\mathrm{min}}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\dlyap}{\mathsf{dlyap}}
\renewcommand{\vec}{\mathrm{vec}}
\newcommand{\bigopnorm}[1]{\bignorm{#1}_{\mathrm{op}}}
\newcommand{\mat}{\mathrm{mat}}

\newcommand{\vfapprox}{V_{\phi,w}}
\newcommand{\vfhatapprox}{V_{\phi,\hat w}}
\newcommand{\vfoptapprox}{V_{\phi,w^*}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathscr{N}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\rE}{\mathbb{E}}
\newcommand{\rI}{\mathbb{I}}
\newcommand{\rM}{\mathbb{M}}
\newcommand{\rN}{\mathbb{N}}
\newcommand{\rP}{\mathbb{P}}
\newcommand{\rR}{\mathbb{R}}
\newcommand{\rT}{\mathbb{T}}

\newcommand{\weights}{\omega}

\newcommand{\Pperpphi}{P^\perp_{\Phi}}

\newcommand{\Rmin}{R_{\textrm{min}}}
\newcommand{\Rmax}{R_{\textrm{max}}}
\newcommand{\Vmax}{V_{\textrm{max}}}
\newcommand{\rpi}{r_\pi}
\newcommand{\Ppi}{P_\pi}

\newcommand{\rad}{\operatorname{Rad}}
\newcommand{\hH}{\hat{\mathcal{H}}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\expect}{{\huge \mathbb{E}}}
\newcommand{\expects}{\expect\nolimits}

\newcommand{\rank}{\text{Rank}}
\newcommand{\spn}{\text{Span}}

\newcommand{\mdp}{\mathcal{M}}
\newcommand{\sspace}{\mathcal{S}}
\newcommand{\rew}{\mathcal{R}}
\newcommand{\prob}{\mathcal{P}}
\newcommand{\trans}{\mathcal{T}}
\newcommand{\aspace}{\mathcal{A}}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}

\newcommand{\cbar}{\, | \,}
\newcommand{\cdbar}{\, \| \,}
\newcommand{\csemi}{\, ; \,}

\newcommand{\charline}[1]{\textcolor{red}{[Charline: #1]}}
\newcommand{\marc}[1]{\textcolor{pink}{[Marc: #1]}}
\newcommand{\rishabh}[1]{{\textcolor{blue}{Rishabh: #1}}}
\newcommand{\markcomment}[2][]{\todo[size=\tiny,color=black!20!white,#1]{\textbf{Mk: } #2}\xspace}

\usepackage{xspace}
\usepackage[textsize=tiny,
]{todonotes}

\iftrue
\renewcommand{\charline}[2][]{\todo[size=\tiny,color=red!20!white,#1]{\textbf{C: } #2}\xspace}
\renewcommand{\marc}[2][]{\todo[size=\tiny,color=pink!20!white,#1]{\textbf{M: } #2}\xspace}
\renewcommand{\rishabh}[2][]{\todo[size=\tiny,color=blue!20!white,#1]{\textbf{R: } #2}\xspace}
\renewcommand{\markcomment}[2][]{\todo[size=\tiny,color=black!20!white,#1]{\textbf{Mk: } #2}\xspace}
\setlength{\marginparwidth}{22ex}
\fi
